Statistics of BY Draconis Chromospheric Variable Stars

We present an extensive catalogue of BY Draconis (BY Dra)-type variables and their stellar parameters. BY Dra are main-sequence FGKM-type stars. They exhibit inhomogeneous starspots and bright faculae in their photospheres. These features are caused by stellar magnetic fields, which are carried along with the stellar disc through rotation and which produce gradual modulations in their light curves (LCs). Our main objective is to characterise the properties of BY Dra variables over a wide range of stellar masses, temperatures and rotation periods. A recent study categorised 84,697 BY Dra variables from Data Release 2 of the Zwicky Transient Facility based on their LCs. We have collected additional photometric data from multiple surveys and performed broad-band spectral energy distribution fits to estimate stellar parameters. We found that more than half of our sample objects are of K spectral type, covering an extensive range of stellar parameters in the low-mass regime (0.1-1.3 M$_{\odot}$ ). Compared with previous studies, most of the sources in our catalogue are rapid rotators, and so most of them must be young stars for which a spin-down has not yet occurred. We subdivided our catalogue based on convection zone depth and found that the photospheric activity index, $S_{\rm ph}$, is lower for higher effective temperatures, i.e., for thinner convective envelopes. We observe a broad range of photospheric magnetic activity for different spectral classes owing to the presence of stellar populations of different ages. We found a higher magnetically active fraction for K- than M-type stars.

==> Statistical Study of BY Draconis Chromospheric Variable Stars/Table1.tex <==
%\begin{landscape}
\begin{table*}
\caption{LC data from \citet{Chen2020} combined with photometric data of BY Dra variable candidates from multiple surveys.}
\centering
%\tabletypesize{1pt}
\setlength{\tabcolsep}{1pt}
\resizebox{1\textwidth}{!}{%
\begin{tabular}{@{}cccccccccccccccccccc@{}}
\hline
\hline
ID & \begin{tabular}[c]{@{}c@{}} RA (J2000)\\ (deg)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Dec (J2000)\\ (deg)\end{tabular} & \begin{tabular}[c]{@{}c@{}} Parallax\\ (mas)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Distance\\ (pc)\end{tabular} & \begin{tabular}[c]{@{}c@{}}$\langle g \rangle$\\ (mag)\end{tabular} & \begin{tabular}[c]{@{}c@{}}$\langle r \rangle$\\ (mag)\end{tabular} & \begin{tabular}[c]{@{}c@{}}$\langle G \rangle$\\ (mag)\end{tabular} & \begin{tabular}[c]{@{}c@{}}$\langle BP \rangle$\\ (mag)\end{tabular} & \begin{tabular}[c]{@{}c@{}}$\langle RP \rangle$\\ (mag)\end{tabular} & \begin{tabular}[c]{@{}c@{}}$\langle J \rangle$\\ (mag)\end{tabular} & \begin{tabular}[c]{@{}c@{}}$\langle H \rangle$\\ (mag)\end{tabular} & \begin{tabular}[c]{@{}c@{}}$\langle K \rangle$\\ (mag)\end{tabular} & \begin{tabular}[c]{@{}c@{}}$\langle W1 \rangle$\\ (mag)\end{tabular} & \begin{tabular}[c]{@{}c@{}}$\langle W2 \rangle$\\ (mag)\end{tabular} & ... & \begin{tabular}[c]{@{}c@{}}Period\\ (days)\end{tabular} & \begin{tabular}[c]{@{}c@{}} Amp$_{g}$\\ (mag)\end{tabular} & \begin{tabular}[c]{@{}c@{}} Amp$_{r}$\\ (mag)\end{tabular} & ... \\ \hline
ZTFJ000000.13+620605.8 & 0.00056 & 62.10163 & 1.58 & 636.77 & 16.79 & 15.73 & 15.77 & 16.56 & 14.95 & 13.83 & 13.24 & 13.06 & --- & --- & ... & 1.945 & 0.113 & 0.078 & ... \\
ZTFJ000002.20+480720.8 & 0.00918 & 48.12246 & 1.96 & 510.07 & 16.87 & 15.81 & 15.88 & 16.60 & 15.06 & 14.04 & 13.41 & 13.25 & 13.18 & 13.19 & ... & 0.381 & 0.107 & 0.093 & ... \\
ZTFJ000003.23+543605.4 & 0.01347 & 54.60151 & 1.15 & 846.92 & 17.20 & 16.22 & 16.33 & 17.03 & 15.52 & 14.45 & 13.73 & 13.73 & 13.56 & 13.63 & ... & 0.786 & 0.166 & 0.112 & ... \\
ZTFJ000003.76+532917.1 & 0.01568 & 53.48811 & 0.89 & 1116.84 & 15.84 & 15.32 & 15.35 & 15.73 & 14.79 & 14.20 & 13.74 & 13.59 & 13.66 & 13.66 & ... & 0.592 & 0.164 & 0.159 & ... \\
ZTFJ000004.34+522031.5 & 0.01809 & 52.34209 & 0.92 & 1078.8 & 17.04 & 16.28 & 16.41 & 16.94 & 15.73 & 14.98 & 14.32 & 14.26 & 14.16 & 14.22 & ... & 4.083 & 0.087 & 0.095 & ... \\
... & ... & ... &  &  & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ...  \\
... & ... & ... &  &  & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... \\ \hline
\end{tabular}%
}
\label{table1}
\end{table*}
%\end{landscape}


==> Statistical Study of BY Draconis Chromospheric Variable Stars/Table2.tex <==

%\begin{landscape}
\begin{table*}
\caption{Stellar Parameters of our sample BY Dra variable candidates}
\centering
\setlength{\tabcolsep}{1pt}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}ccccccccccccccccc@{}}
\hline
\hline
$\rm {ID}$ & \begin{tabular}[c]{@{}c@{}}RA \ (J2000)\\ (deg)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Dec (J2000)\\ (deg)\end{tabular} & ... & \begin{tabular}[c]{@{}c@{}}$T_{\rm eff}$\\ (K)\end{tabular} & \begin{tabular}[c]{@{}c@{}}$\log g$\\ (cm s$^{-2}$)\end{tabular} & $\chi_{\rm red}^{2}$ & \begin{tabular}[c]{@{}c@{}}Luminosity\\ (L$_{\odot}$)\end{tabular} & \begin{tabular}[c]{@{}c@{}} $\pm$\\ (L$_{\odot}$)\end{tabular} & \begin{tabular}[c]{@{}c@{}} Radius\\ (R$_{\odot}$)\end{tabular} & \begin{tabular}[c]{@{}c@{}}$\pm$\\ (R$_{\odot}$)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Mass\\ (M$_{\odot})$\end{tabular} & \begin{tabular}[c]{@{}c@{}}...\\ \end{tabular} & \begin{tabular}[c]{@{}c@{}}Age\\ (Gyr)\end{tabular} & \begin{tabular}[c]{@{}c@{}}...\\ \end{tabular} & \begin{tabular}[c]{@{}c@{}}$S_{{\rm ph},g}$\\ ($\rm ppm$)\end{tabular} &
\begin{tabular}[c]{@{}c@{}}$S_{{\rm ph},r}$\\ ($\rm ppm$)\end{tabular} \\ \hline
ZTFJ000000.13+620605.8 & 0.00056 & 62.10163 & ... & 4200 & 4.5 & 9.82 & 0.215 & 0.014 & 0.87 & 0.025 & 0.8 & ... & 0.03 & ... & 2121 & 1406 \\
ZTFJ000002.20+480720.8 & 0.00918 & 48.12246 & ... & 4300 & 5 & 8.65 & 0.117 & 0.005 & 0.61 & 0.01 & --- & ... & --- & ... & --- & --- \\
ZTFJ000003.23+543605.4 & 0.01347 & 54.60151 & ... & 4200 & 2.5 & 5.15 & 0.224 & 0.018 & 0.90 & 0.03 & 0.81 & ... & 0.028 & ... & 3104 & 2324 \\
ZTFJ000003.76+532917.1 & 0.01568 & 53.48811 & ... & 5400 & 4.5 & 6.01 & 0.694 & 0.04 & 0.95 & 0.02 & 0.91 & ... & 0.037 & ... & 3056 & 2847 \\
ZTFJ000003.34+522031.5 & 0.01809 & 52.34209 & ... & 4700 & 3.5 & 2.95 & 0.278 & 0.032 & 0.795 & 0.043 & 0.78 & ... & 0.05 & ... & 2037 & 1438 \\
... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ...\\
... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ... & ...\\ \hline
\end{tabular}%

}
\label{table2}
\end{table*}
%\end{landscape}
